One Model to Synthesize Them All: Multi-contrast Multi-scale Transformer for Missing Data Imputation

Multi-contrast magnetic resonance imaging (MRI) is widely used in clinical practice as each contrast provides complementary information. However, the availability of each imaging contrast may vary amongst patients, which poses challenges to radiologists and automated image analysis algorithms. A general approach for tackling this problem is missing data imputation, which aims to synthesize the missing contrasts from existing ones. While several convolutional neural networks (CNN) based algorithms have been proposed, they suffer from the fundamental limitations of CNN models, such as the requirement for fixed numbers of input and output channels, the inability to capture long-range dependencies, and the lack of interpretability. In this work, we formulate missing data imputation as a sequence-to-sequence learning problem and propose a multi-contrast multi-scale Transformer (MMT), which can take any subset of input contrasts and synthesize those that are missing. MMT consists of a multi-scale Transformer encoder that builds hierarchical representations of inputs combined with a multi-scale Transformer decoder that generates the outputs in a coarse-to-fine fashion. The proposed multi-contrast Swin Transformer blocks can efficiently capture intra- and inter-contrast dependencies for accurate image synthesis. Moreover, MMT is inherently interpretable as it allows us to understand the importance of each input contrast in different regions by analyzing the in-built attention maps of Transformer blocks in the decoder. Extensive experiments on two large-scale multi-contrast MRI datasets demonstrate that MMT outperforms the state-of-the-art methods quantitatively and qualitatively.

==> sections/acknowledgement.tex <==
\section{Acknowledgement}

==> sections/background.tex <==
\section{Background}
\subsection{Scaled dot-product attention}
The core of Transformer~\cite{NIPS2017_3f5ee243} is self-attention, which is a differentiable module that maps a query along with some key-value pairs to an output. The output is effectively the weighted sum of the given values and the weights are defined by a compatibility function that maps queries to its corresponding keys. For a given query $Q$, key $K$ and value $V$, the scaled dot-product attention proposed by~\cite{NIPS2017_3f5ee243} is defined as 

\begin{equation}
    \text{Attention}(Q, K, V) = \text{softmax}(\frac{QK^T}{\sqrt{d_k}})V
    \label{eq1}
\end{equation}

where $Q \in \mathbb{R}^{M \times d_k}$, $K \in \mathbb{R}^{N \times d_k}$ and $V \: \in \mathbb{R}^{N \times d_v}$. 

\subsection{Multi-head attention}
Multi-head attention (MHA)~\cite{NIPS2017_3f5ee243} is a parallel operation wherein multiple scaled-dot product attention operations are performed $h$ times, where $Q$, $K$ and $V$ are linearly projected with multiple learned linear projections. MHA enables the model to jointly pay attention to information from different subspace representations at various different input positions. 
\begin{equation}
    \text{MHA}(Q, K, V) = \text{Concat}(\text{head}_1, ..., \text{head}_h)W^O
    \label{eq2}
\end{equation}

where $\text{head}_i = \text{Attention}(QW_i^Q, KW_i^K, VW_i^V)$ and the projections are parameterized by matrices $W_i^Q \in \mathbb{R}^{d_{model} \times d_k}$,  $W_i^K \in \mathbb{R}^{d_{model} \times d_k}$ and $W_i^V \in \mathbb{R}^{d_{model} \times d_v}$.

\subsection{Swin Transformer}
The computational complexity of self-attention is quadratic to image size, which makes it intractable for Transformer on high-resolution images. To overcome this, Liu \etal~\cite{swin} proposed Swin Transformer where self-attention is computed locally within non-overlapping local and the window partition are shifted between consecutive self-attention layers. The shifted windowing scheme achieves linear computational complexity with respect to the image size, while also allows cross-window connection. In addition, the Swin Transformer has a hierarchical architecture that enables flexible representation of images at various scales, which is important for vision tasks.
